Distance Oracles for Interval Graphs via Breadth-First Rank/Select in Succinct Trees

We present the first succinct distance oracles for (unweighted) interval graphs and related classes of graphs, using a novel succinct data structure for ordinal trees that supports the mapping between preorder (i.e., depth-first) ranks and level-order (breadth-first) ranks of nodes in constant time. Our distance oracles for interval graphs also support navigation queries -- testing adjacency, computing node degrees, neighborhoods, and shortest paths -- all in optimal time. Our technique also yields optimal distance oracles for proper interval graphs (unit-interval graphs) and circular-arc graphs. Our tree data structure supports all operations provided by different approaches in previous work, as well as mapping to and from level-order ranks and retrieving the last (first) internal node before (after) a given node in a level-order traversal, all in constant time.

==> preamble.tex <==
\makeatletter
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{slantsc}

\usepackage{babel}
\input{ushyphex.tex} % hyphenation exceptions


\newcommand{\ifarxiv}[2]{\ifthenelse{\equal{\version}{arxiv}}{#1}{#2}}
\newcommand{\ifconf}[2]{\ifthenelse{\equal{\version}{conference}}{#1}{#2}}

\usepackage{array,multicol}
\usepackage{amsmath,amsfonts,amssymb,mathtools}
\usepackage{mleftright}\mleftright % redefine left and right to not add space around braces
\usepackage{relsize,ifthen,xspace,enumitem,booktabs,adjustbox,needspace,pbox}
\usepackage{graphicx}



%
%
%
%
%
%


\usepackage{wref}
\usepackage[bibtex]{url-doi-arxiv}




%%
%
%
%
%
%

%
%
%
%
%%
%%
%%
%%
%%
%%
%%
%%
%
%
%
%
%%
%
%
%
%
%
%
%
%%
%
%


%
%\usepackage{pdflscape} % use this instead to rotate pdf pages.


%Helper macros

\newcommand\plaincenter[1]{%
	\mbox{}\hfill#1\hfill\mbox{}%
}
\newcommand\plaincenterbox[1]{%
	\mbox{}\hfill\mbox{#1}\hfill\mbox{}%
}













\usepackage{tikz}
\usepackage{relsize}
\usetikzlibrary{positioning,arrows.meta}
\usetikzlibrary{backgrounds,calc,trees}

\pgfdeclarelayer{background}
\pgfsetlayers{background,main}


% Make title and author accessible in document
\AtBeginDocument{%
	\let\mytitle\@title%
}



%
%
%
%%
%
%
%
%
%
%
%
%
%
%
%%
%
%
%
%



\hypersetup{
	final,
	unicode=true, 
	bookmarks=true,
	bookmarksnumbered=true,
	bookmarksdepth=2,
	bookmarksopen=true,
	breaklinks=true,
	hidelinks,
	pdfhighlight={/P}
}



% Theorems etc
%\iflipics{
	\newtheorem{fact}[theorem]{Fact}
%}{}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\newenvironment{thmenumerate}[2][]{%
	\begin{enumerate}[
%
		label={\textsf{\textbf{\color{darkgray}{\makebox[\widthof{(a)}][c]{\textup{(\alph*)}}}}}},
		ref={\ref{#2}\kern.1em--\kern.1em(\alph*)},
		itemsep=0pt,
		topsep=.5ex,
		leftmargin=1.75em,
		#1
	]%
}{%
	\end{enumerate}%
}




%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
















%    __  __                          
%   |  \/  | __ _  ___ _ __ ___  ___ 
%   | |\/| |/ _` |/ __| '__/ _ \/ __|
%   | |  | | (_| | (__| | | (_) \__ \
%   |_|  |_|\__,_|\___|_|  \___/|___/
%                                    


% Common phrases
\newcommand*\ie{\mbox{i.\hspace{.2ex}e.}}
\newcommand*\eg{\mbox{e.\hspace{.2ex}g.}}
\newcommand*\iid{\mbox{i.\hspace{.2ex}i.\hspace{.2ex}d.}\xspace}
\newcommand*\wrt{\mbox{w.\hspace{.2ex}r.\hspace{.2ex}t.}\xspace}
\newcommand*\aka{\mbox{a.\hspace{.2ex}k.\hspace{.2ex}a.}\xspace}
\newcommand*\withoutlossofgenerality{\mbox{w.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\Withoutlossofgenerality{\mbox{W.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\almostsurely{\mbox{a.\hspace{.2ex}s.}\xspace}
\newcommand*\whp{\mbox{w.\hspace{.2ex}h.\hspace{.2ex}p.}\xspace}


\newcommand\R{\mathbb R}
\newcommand\N{\mathbb N}
\newcommand\Z{\mathbb Z}
\newcommand\Q{\mathbb Q}
\renewcommand\C{\mathbb{C}}
\newcommand\Oh{O}
\def\.{\mskip1mu} 


%



\newcommand{\surroundedmath}[3]{% #1=mathrel/mathbin/etc #2=spacing #3=symbol
	\mathchoice{%display
		#1{#2{#3}#2}%
	}{%text
		#1{#3}%
	}{%script
		#1{#3}%
	}{%scriptsript
		#1{#3}%
	}%
}
\newcommand\rel[1]{\surroundedmath{\mathrel}{\:}{#1}}
\newcommand\wrel[1]{\surroundedmath{\mathrel}{\;}{#1}}
\newcommand\wwrel[1]{\surroundedmath{\mathrel}{\;\;}{#1}}
\newcommand\bin[1]{\surroundedmath{\mathbin}{\:}{#1}}
\newcommand\wbin[1]{\surroundedmath{\mathbin}{\;}{#1}}
\newcommand\wwbin[1]{\surroundedmath{\mathbin}{\;\;}{#1}}

\newcommand{\eqwithref}[2][c]{%
	\relwithref[#1]{#2}{=}%
}
\newcommand{\relwithref}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize\wref{#2}}}}{#3}}%
}
\newcommand{\relwithtext}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize#2}}}{#3}}%
}

\newcommand\pe{\phantom{{}={}}}
\newcommand\ppe{\phantom{=}}


\newcommand{\ESymbol}{\mathbb{E}}
\newcommand{\V}{\ensuremath{\mathrm{Var}}}
\newcommand{\Cov}{\ensuremath{\mathrm{Cov}}}
\newcommand{\ProbSymbol}{\ensuremath{\mathbb{P}}}
\providecommand{\given}{}
%% mathtools command to declare cool delimiter pairs:
%	\DeclarePairedDelimiterXPP{cmd}[numargs]{pre code}{left_delim}{right_delim}{post code}{body}
\DeclarePairedDelimiterXPP\Prob[1]{\ProbSymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\DeclarePairedDelimiterXPP\E[1]{\ESymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\DeclarePairedDelimiterXPP\Eover[2]{\ESymbol_{#1}}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#2%
}
\providecommand{\Prob}{} % hack for syntax highlighting ...
\providecommand{\E}{} % hack for syntax highlighting ...
\providecommand{\Eover}{} % hack for syntax highlighting ...









\newcommand\idtt[1]{\texttt{\upshape #1}\xspace}

%bit vectors
\def\rankop{\idtt{rank}}
\def\selop{\idtt{select}}
\def\accessop{\idtt{access}}

%%%% Orders
\def\DFUDS{\idtt{DFUDS}}
\def\LOUDS{\idtt{LOUDS}}
\def\BP{\idtt{BP}}
\def\PB{\idtt{PB}}
\def\TC{\idtt{TC}}
\def\pre{\idtt{PRE}}
\def\post{\idtt{POST}}
\def\inorder{\idtt{IN}}
\def\lvl{\idtt{LEVEL}}


%trees
\def\TrParent{\idtt{parent}}
\def\TrChild{\idtt{child}}
\def\TrLastChild{\idtt{last\_child}}
\def\TrDepth{\idtt{depth}}
\def\TrLevAnc{\idtt{anc}}
\def\TrRank{\idtt{node\_rank}}
\def\TrSelect{\idtt{node\_select}}
\def\TrChildRank{\idtt{child\_rank}}
\def\TrDeg{\idtt{degree}}
\def\TrNbDesc{\idtt{nbdesc}}
\def\LCA{\idtt{LCA}}
\def\TrHeight{\idtt{height}}
\def\TrDistance{\idtt{distance}}
\def\TrLeftLeaf{\idtt{leftmost\_leaf}}
\def\TrRightLeaf{\idtt{rightmost\_leaf}}
\def\TrLeafSize{\idtt{leaf\_size}}
\def\TrLeafRank{\idtt{leaf\_rank}}
\def\TrLeafSel{\idtt{leaf\_select}}
\def\TrLevelLeft{\idtt{level\_leftmost}}
\def\TrLevelRight{\idtt{level\_rightmost}}
\def\TrLevelSucc{\idtt{level\_succ}}
\def\TrLevelPred{\idtt{level\_pred}}
\def\TrPrevInt{\idtt{prev\_internal}}
\def\TrNextInt{\idtt{next\_internal}}
\def\TrHeight{\idtt{height}}



%graphs
\def\GDegree{\idtt{degree}}
\def\GAdjacent{\idtt{adjacent}}
\def\GNeighbor{\idtt{neighborhood}}
\def\GSPath{\idtt{spath}}
\def\GDistance{\idtt{distance}}

















% Make align suppress number for \\* lines
% define galign to use subequation labels
\makeatletter
\let\oldalign\align
\let\endoldalign\endalign

\newcommand*\numberthis[1][]{\stepcounter{equation}\tag{\theequation}}

%\iflipics{}{
	\renewenvironment{align}{%
		\begingroup%
		\let\oldhalign\halign
		\def\halign{%
			\let\oldbreak\\%
			\def\nonnumberbreak{\nonumber\oldbreak*}%
			\def\\{%
				\@ifstar{\nonnumberbreak}{\oldbreak}%
			}%
			\oldhalign%
		}
		\let\oldlabel\label%
		\oldalign%
	}{%
		\endoldalign%
		\endgroup%
	}
%}

\newenvironment{galign}[1][]{%
	\subequations%
	#1%
%
	\def\theequation{\theparentequation{\protect\footnotesize\hspace{.1em}.\arabic{equation}}}%
%
	\align%
}{%
	\endalign%
	\endsubequations%
}

%http://tex.stackexchange.com/a/309558
\newcommand\splitaftercomma[1]{%
  \begingroup
  \begingroup\lccode`~=`, \lowercase{\endgroup
    \edef~{\mathchar\the\mathcode`, \penalty0 \noexpand\hspace{0pt plus .25em}}%
  }\mathcode`,="8000 #1%
  \endgroup
}


\newcommand\tagref[2][\width]{%
	\tag*{\makebox[#1][r]{\wref{#2} \scriptsize revisited}}%
}


\newcommand\separatedpar{%
	\medskip
	\plaincenter{%
		$*$\hspace{3em}$*$\hspace{3em}$*$%
	}\par
	\medskip
	\noindent
}


% Notation list
\def\mydots{\xleaders\hbox to.5em{\hfill.\hfill}\hfill}


\newlength\tmpLenNotations
\newenvironment{notations}[1][10em]{%
	\small
	\newcommand\notationentry[1]{%
		\settowidth\tmpLenNotations{##1}%
		\ifthenelse{\lengthtest{\tmpLenNotations > \labelwidth}}{%
			\parbox[b]{\labelwidth}{%
				\makebox[0pt][l]{##1}\\%
			}%
		}{%
			\mbox{##1}%
		}%
		\mydots\relax%
	}%
	\begin{list}{}{%
		\setlength\labelsep{0em}%
		\setlength\labelwidth{#1}%
		\setlength\leftmargin{\labelwidth+\labelsep+1em}%
		\renewcommand\makelabel{\notationentry}%
	}
	\ifdraft{%
		\newcommand\notation[1]{%
			\item[{##1}] \marginpar{%
				\adjustbox{scale={.55}{1},outer}{%
					\color{brown!80}%
					\scriptsize$\triangleright$\;\tiny\texttt{\detokenize{##1}}%
				}%
			}%
		}%
	}{%
		\newcommand\notation[1]{\item[{##1}]}%
	}%
	\raggedright
}{%
	\end{list}
}
\newcommand*\phdthesis{\mbox{Ph.\hspace{.2ex}D.} thesis\xspace}


%%%%% Allow page breaks in display math environments 
%%%%% With this, display environments can be broken as paragraphs.
%%%%% The 1 means that such breaks should be considered not nice, but acceptable.
\allowdisplaybreaks[3]

%
%
%
%
%
%
%
%
%
%
%

% !BIB program = bibtex
%\bibliographystyle{plainurl} % already set by url-doi-arxiv

\let\oldthebibliography\thebibliography
\renewcommand\thebibliography[1]{%
	\oldthebibliography{#1}%
	\pdfbookmark[1]{References}{}%
%
%
}


%
%
%
%





%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%\ifdraft{}{%
	\usepackage{microtype}
%}

\let\epsilon\varepsilon


\newsavebox\tmpbox

\raggedbottom


%
%
%
%
%
%



%
%
%
%%
%
%


\makeatother


